Retrieval-Augmented Generation for Code Summarization via Hybrid GNN

Source code summarization aims to generate natural language summaries from structured code snippets for better understanding code functionalities. However, automatic code summarization is challenging due to the complexity of the source code and the language gap between the source code and natural language summaries. Most previous approaches either rely on retrieval-based (which can take advantage of similar examples seen from the retrieval database, but have low generalization performance) or generation-based methods (which have better generalization performance, but cannot take advantage of similar examples). This paper proposes a novel retrieval-augmented mechanism to combine the benefits of both worlds. Furthermore, to mitigate the limitation of Graph Neural Networks (GNNs) on capturing global graph structure information of source code, we propose a novel attention-based dynamic graph to complement the static graph representation of the source code, and design a hybrid message passing GNN for capturing both the local and global structural information. To evaluate the proposed approach, we release a new challenging benchmark, crawled from diversified large-scale open-source C projects (total 95k+ unique functions in the dataset). Our method achieves the state-of-the-art performance, improving existing methods by 1.42, 2.44 and 1.29 in terms of BLEU-4, ROUGE-L and METEOR.

==> approach.tex <==
% We first give a formal formulation of this task, then present each component in details.


\begin{figure*}[t]
     \centering
     \includegraphics[width=0.95\textwidth, height=6cm]{images/nips_overview_cropped.pdf}
     \vspace{-2mm}
     \caption{The framework of our \textit{FusionGNN}. Best viewed in color.} 
     \label{fig:framework}
     \vspace{-2mm}
\end{figure*}

%\subsection{Problem Formulation}
In this section, we introduce our proposed ~\textit{FusionGNN} framework, as shown in Figure~\ref{fig:framework}, which mainly includes four components: 1) Semantic-based Graph Construction, which encodes the source code of a function into a code property graph with a novel semantic-augmented mechanism by retrieving the similar code in the retrieval code database to augment code semantics. 2) Attention-based Dynamic Graph Construction, which dynamically constructs a graph to capture the global relations among nodes. 3) Hybrid Message Passing (HMP)-GNN Encoder, which fuses the messages from the constructed semantic-based graph and attention-based graph to learn comprehensive code semantics. 4) Decoder, which utilizes an attention-based BiLSTM to generate a summary.

\subsection{Problem Formulation}
In this work, we focus on generating summaries for functions~\cite{wan2018improving,zhangretrieval}.
We define a dataset as $D = \{(c, s)| c \in C, s \in S\}$, where $c$ is a source code in the function set $C$, $s$ represents its targeted summary in $S$. The task of code summarization is to generate the best summary consisting of a sequence of tokens with $T$ length $\hat{S}=\{s_1, s_2,...,s_T\}$ which maximize the conditional likelihood $\hat{S} = \mathrm{argmax}_S P(S| C)$.



\subsection{Semantic-based Static Graph Construction} \label{sec:static}
\subsubsection{Code Property Graph}
%In this part, we propose to fuse diverse dimensional semantics ({e.g.,} AST, CFG and PDG) into Code Property Graph (CPG) and introduce our well-designed semantic-augmented mechanism to augment code semantics.

We leverage the Code Property Graph (CPG)~\cite{yamaguchi2014modeling} to combine diverse graph representations (i.e., AST, CFG, and PDG) into a single graph structure. Thus, CPG could capture comprehensive semantics of a program from different perspectives. For more details on CPG with a simple example, please refer to Appendix~\ref{sec:cpg}. Here we describe each representation briefly as follows:

% Yamaguchi et al.~\cite{yamaguchi2014modeling} proposed Code Property Graph (CPG) to combine several graph representations (e.g., AST, CFG, and PDG) into a single graph structure, which is shown in Figure~\ref{fig:graph_representation}. We follow this definition and explain each type of representations as follows:

\begin{itemize}[leftmargin=*]
  \item \textbf{Abstract Syntax Tree (AST).} 
  AST is a representation of the abstract syntactic structure of source code, which omits irrelevant details that have no effect on the semantics. Each node in AST is constituted by node type i.e., \textit{identifier}, \textit{callee} and the subsequence i.e., ``\textit{a++}'' from the source code ``\textit{int b = a++}''.
%   Figure.~\ref{fig:graph_representation} shows the completed AST nodes on the left simple program and each node has a code sequence in the first line and type attribute in the second line. The black arrows represent the child-parent relations among ASTs. 
  \item \textbf{Control Flow Graph (CFG).} Compared with AST highlighting the syntactic structure, CFG displays statement execution order,  {i.e.,} the possible order in which statements may be executed and the conditions that must be met for this to happen. Each statement in the program is treated as an independent node as well as a designated entry and exit node. Based on the keywords \textit{if}, \textit{for}, \textit{goto}, \textit{break} and \textit{continue}, control flow graphs can be easily built and ``Flow to '' edge describes this flow order between statements.
%   and ``Flow to'' with green dashed arrows in Figure~\ref{fig:graph_representation} represents this flow order.
  \item \textbf{Program Dependency Graph (PDG).} PDG includes \textbf{data dependencies} and \textbf{control dependencies}: 1) data dependencies are described as the definition of a variable in a statement reaches the usage of the same variable at another statement. 
  For example, a variable ``\textit{b}'' is defined in the statement ``\textit{int b = a++}'' and used in ``\textit{call (b)}''. Hence, there is a ``Reach'' edge points from ``\textit{int b = a++}'' to ``\textit{call (b)}''.
  Furthermore, ``Define/Use'' edge 
%   with orange double arrows
  denotes the definition and usage of the variable. 
  2) different from CFG displaying the execution process of the complete program, control dependencies define the execution of a statement may be dependent on the value of a predicate. 
  For instance, suppose there are two statements ``\textit{int b = a++}'' and ``\textit{call (b)}'' that are only performed when ``\textit{a}'' is even. Then, a ``Control'' edge points from ``\textit{if (a \% 2) == 0}'' to ``\textit{int b = a++}'' and ``\textit{call (b)}''.
\end{itemize}
Formally, one raw function $c$ could be represented by a multi-edged CPG $g(V,\boldsymbol A)$. Let $m$ be the total number of nodes in $V$, $\boldsymbol A \in \{0,1\}^{k \times m \times m }$ is the adjacency matrix, where $k$ is the total number of edge types. An element $a^{e}_{i,j} \in \boldsymbol A$ equal to $1$ indicates that node $v_i, v_j$ is connected via an edge of type $e$, and $0$ otherwise.



% As compared to LeClair et al.~\cite{leclair2020improved}, we encode diverse dimensional semantics~{e.g.,} CFG, PDG into the code property graph (CPG). The difference from Zhou et al.~\cite{zhou2019devign} is that we combine DFG\_R and DFG\_W into single edge Define/Use and encode more edge types (e.g., control dependencies).
\subsubsection{Node Initialization Representation}
%Some works~\cite{zhou2019devign, allamanis2017learning} utilize random or Word2Vec embedding for nodes, however,
The nodes in CPG are represented by node type and their subsequences. To better capture the dependency in the subsequence, we utilize a BiLSTM to initialize the node. We first embed the node type into label embedding, ~\textit{i.e.,} each node type is assigned a unique integer $h_{type}$. Then a BiLSTM is used to encode the subsequence within the node. Specifically, for a node $v \in V$, its subsequence is defined as $S_v = \{s_{v,1}, s_{v,2},..., s_{v,l}\}$ where $l$ is the length of sequence. Each $\boldsymbol s_{v,i}$ is embedded with a learnt embedding matrix $\boldsymbol E$ and we use a BiLSTM to encode $S_v$ to get the final states $\boldsymbol h_{seq}$. Finally, we concatenate node type representation with sequence representation and employ a linear projection to represent node feature $\boldsymbol h_v$. The initial node feature $\boldsymbol h_v \in \boldsymbol H$ can be expressed as follows:
\begin{small}
\begin{align}
% \mathrm{BiLSTM}(\boldsymbol E(s_{v,1}),...,\boldsymbol E(s_{v,l}))
\boldsymbol h_{v,1},...,\boldsymbol h_{v,l} = \mathrm{BiLSTM}(\boldsymbol E_{v,1},...,\boldsymbol E_{v,l}) & &\boldsymbol h_{\mathrm{seq}} = [\boldsymbol h_{v,1}^\rightarrow;\boldsymbol h_{v,l}^\leftarrow] &&\boldsymbol h_{v} = \mathrm{linear}(\mathrm{concat}[h_{type}; \boldsymbol h_{seq}])
\end{align}
\end{small}
By node initialization, $g(V,\boldsymbol A)$ can be expressed as $g(V,\boldsymbol H,\boldsymbol A)$, where $\boldsymbol H \in \mathbb{R}^{m \times d} $ is the initial node feature matrix and each vertex $v$ in $V$ is represented by a $d$-dim real-valued vector  $\boldsymbol h_v  \in \mathbb{R}^d$. 


\subsubsection{Semantic-augmented Mechanism} \label{sec:retrieved-code}
Suppose there is a CPG $g(V_c,\boldsymbol H_c,\boldsymbol A_c)$ of source code $c$, our goal is to learn a function $f$ to generate $s= f(g(V_c,\boldsymbol H_c,\boldsymbol A_c))$, however, due to the complexity of learning code semantics, $f$ is hard to learn. Our novel semantic-augmented mechanism is motivated that for another known code-summary pair $(c',s')$ satisfies $s'=f(g(V_{c'},\boldsymbol H_{c'},\boldsymbol A_{c'}))$, where $c$ and $c'$ are similar. A simple linear transformation can be performed $s=f(g(V_c,\boldsymbol H_c,\boldsymbol A_c)) - f(g(V_{c'},\boldsymbol H_{c'},\boldsymbol A_{c'})) + s'$. Compared to learn $f$ directly from $g(V_c,\boldsymbol H_c,\boldsymbol A_c)$ to $s$, if we can make full use of $f(g(V_{c'},\boldsymbol H_{c'},\boldsymbol A_{c'}))$ and $s'$, it can be regraded as a well supplementary for original $c$ to learn the comprehensive semantics. Based on this, our novel semantic-augmented mechanism is performed with three steps:

% CPG encodes diverse program representations, however, it is not easy to learn the comprehensive semantics of programs directly.
% Thus, to better learn semantics, we propose a novel semantic-augmented mechanism that adds the retrieval semantics into the original CPG. For each training data $c$, we first retrieval another program $c'$ that is the most similar to $c$. Then we construct a semantic-augment graph by combining the CPG of $c$, the CPG of $c'$ and the retrieved summary of $c'$ together. Specifically, the static graph is constructed with three steps:

% add more information in the original CPG.

% the original training data such that the semantics could be better learned form the graph.

% to further enrich program semantics, we design our semantic-augmented mechanism, including three components 1) Code Retriever 2) Comp-graph 3) Retrieved Summary Encoder, to augment the retrieved semantics into source code.

\textbf{Step 1: Code Retriever.} For each training sample $(c, s)\in D$, we retrieve the most similar sample: $(c', s')= \mathrm{argmax}_{(c',s')\in D'} cos\_sim(c, c')$, where $c \neq c'$, $D'$ is a given retrieval database and $cos\_sim(c, c')$ is the cosine similarity function. Following Liu et al.~\cite{liu2018neural}, we treat the raw source code $c$ as a ``bag of words'' (BOW) vector and calculate the cosine similarity between the source code $c$ and the retrieved code $c'$ (i.e., $cos\_sim{(c, c')}$ ). 

%$(C', S')$ with the retrieval function $r$: $(c', s')= r(c, C)$, where $c'\in C' \wedge s'\in S' \wedge c\neq c'$. 
% For the retrieval function, following Liu et al.~\cite{liu2018neural}, we treat the raw source code $c$ as a "bag of words" (BOW) vector and retrieve the most similar (Top1) code $c'$ based on the cosine similarity $sim_{(c, c')}$ between the source code $c$ and the retrieved code $c'$ from the training set $C$. 
%Note that we also use code retriever in the training set. 

%For the retrieval function, following Liu et al.~\cite{liu2018neural}, we treat the raw source code $c$ as a "bag of words" (BOW) vector and retrieve the most similar (Top1) code-summary pair $(r_c, r_s)$ based on the cosine similarity $sim_{(c, r_c)}$ between the source code and the retrieved code from the training set. Note that we also use code retriever in the training set. 



\textbf{Step 2: Complementary Graph.}\label{sec:comp-graph}
After retrieving the source code $c'$ for the training sample $c$, we get their corresponding CPGs $g(V_c,\boldsymbol H_c,\boldsymbol A_c)$ and $g(V_{c'},\boldsymbol H_{c'},\boldsymbol A_{c'})$. Then we build a complementary graph by injecting the retrieved graph into the graph of the training sample.
%From Code Retriever, we get a source-retrieved code pair $(c,r_c)$  and the corresponding CPG $g_c(V,\boldsymbol H,\boldsymbol A)$ and $g_r(V,\boldsymbol H,\boldsymbol A)$. We design our comp-graph mechanism to inject retrieved graph semantics into $g_c$. Conceptually, comp-graph consists of three steps: 
\begin{itemize}[leftmargin=*]
  \item 
  To capture the relevance between the two graphs,  we design an attention function, which computes the attention score matrix
  $\boldsymbol A_{i,j}$ for each pair of nodes $v_i\in V_c$ and $v_j\in V_{c'}$:
  %Compute the attention weight $A_{i,j}$ for each pair of node representation $\boldsymbol H_c$ and $\boldsymbol H_{c'}$, we define our attention function as follows:
    \begin{equation}
    \begin{small}
    \boldsymbol A \propto exp(\mathrm{ReLU}(\boldsymbol W \boldsymbol H_c)\mathrm{ReLU}(\boldsymbol W\boldsymbol H_{c'})^T)
    \end{small}
    \end{equation}
    where $\boldsymbol W \in \mathbb{R}^{d \times d} $ are weight matrices with $d$-dim size and ReLU is the rectified linear unit.
  \item Multiply the attention matrix $\boldsymbol A$ with the retrieved node representation $\boldsymbol H_{c'}$ to inject retrieved node features into $\boldsymbol H_{c}$:
    \begin{equation}
    \begin{small}
    \boldsymbol H_c' = z \boldsymbol A \boldsymbol H_{c'}
    \end{small}
    \end{equation}
     where $z=cos\_sim(c,c')$ is the similarity score, which is introduced to weaken the negative impact of $c'$ on $c$, i.e., when the similarity of $c$ and $c'$ is slow.
  \item Finally, we merge $\boldsymbol H_c'$ to the original $\boldsymbol H_{c}$ to get the final node representation.
    \begin{equation}
    \begin{small}
    \boldsymbol {comp} = \boldsymbol W_c\boldsymbol H_c + \boldsymbol W_c'\boldsymbol H_c'
    \end{small}
    \end{equation}
     where $\boldsymbol W_c, \boldsymbol W_c' \in \mathbb{R}^{d \times d} $ are weight matrices and $\boldsymbol {comp}$ is the semantic-augmented node representation, namely \textit{semantic-based static graph}.
     %which is used to compute the static message passing and construct the dynamic graph.
\end{itemize}
\textbf{Step 3: Retrieved Summary Encoder.}
The retrieved summary (i.e., $s'$) may have a semantic overlap with the targeted summary, especially when $c$ and $c'$ are similar. Inspired by the existing work~\cite{yang2019hybrid}, we further encode the semantics of $s'$ with a BiLSTM model i.e., $\{\boldsymbol h_{s'_i}, \forall s'_{i} \in s'\}$ and fuse with the graph encoding results (i.e., the outputs of the GNN encoder) for the decoder, as shown in Figure ~\ref{fig:framework}.

% $\{\boldsymbol h_{s'_i}, \forall s'_{i} \in s'\}$

% To make full use of the retrieved summary $s'$, a simple BiLSTM~\cite{hochreiter1997long} is chosen to compute the sequential output features $\{\boldsymbol h_{s'}, \forall s'_{i} \in s'\}$. Then concatenating with the node representations produced by GNN Encoder in Section~\ref{sec:hybrid} for BiLSTM decoder.




\subsection{Attention-based Dynamic Graph Construction}
% Existing works~\cite{allamanis2017learning,fernandes2018structured,zhou2019devign, hellendoorn2020global} convert code into graph-structured input during preprocessing, and directly consume it via modern neural networks (e.g., GNNs) for computing node and graph embeddings. 
% However, most GNN-based encoders only allow message passing among nodes within a k-hop neighborhood (where k is usually a small number), thus capture only local neighborhood information and ignore global interaction among nodes within the whole graph. 
% This might limit their model capacity of fully encoding the code semantics, especially for a large and complex program.
Due to that GNN-based encoders usually consider the $k$-hop neighborhood, the global relation among nodes in the static graph (see Section~\ref{sec:static}) may be ignored.
In order to better capture the global semantics of source code,  based on the static graph, we propose to dynamically construct a graph via structure-aware global attention mechanism, which allows message passing among any pair of nodes.
We expect this attention-based dynamic graph can better capture the global dependency among nodes, and thus supplement the static graph.

\textbf{Structure-aware Global Attention.}
The construction of the dynamic graph is motivated by the structure-aware self-attention mechanism proposed in~\cite{zhu2019modeling}. 
Given the static graph, we compute a corresponding dense adjacency matrix $\boldsymbol A$ based on a novel structure-aware global attention mechanism and the constructed graph namely \textit{attention-based dynamic graph}. Unlike regular self-attention mechanisms,
we consider not only the node semantics but also the edges in the static graph when computing attention scores between any pair of nodes. We assume that the static graph contains useful structure information which could be utilized for computing the global relationship among nodes.
% Furthermore, in order to force a pair of nodes $(v_i, v_j)$ with edges to have greater attention scores, we apply a ReLU~\cite{nair2010rectified} in our attention mechanism.
\begin{equation}
\begin{small}
    \boldsymbol A_{i,j} = \frac{\mathrm{ReLU}(\boldsymbol h_i \boldsymbol W^Q)(\mathrm{ReLU}(\boldsymbol h_j \boldsymbol W^K)+ \mathrm{ReLU}(\boldsymbol e_{ij} \boldsymbol W^R))}{\sqrt{d}}
\end{small}
\end{equation}
where $\boldsymbol h_i, \boldsymbol h_j \in \boldsymbol {comp}$ are the node representation for any node pair $(v_i, v_j)$, $\boldsymbol e_{ij} \in \mathbb{R}^{d_{e}}$ is the connected edge representation and $\boldsymbol W^Q, \boldsymbol W^K \in \mathbb{R}^{d \times d}$, $\boldsymbol W^R \in \mathbb{R}^{d_{e} \times d}$ are parameter matrices.
We also separate two normalized adjacency matrices $\boldsymbol A^\dashv$ and $\boldsymbol A^\vdash$ from $\boldsymbol A$ according to the incoming/outgoing directions. The dynamic graph $A^\dashv, A^\vdash$ will be used to compute dynamic message passing (see Section~\ref{sec:hybrid}).
\begin{equation}
\begin{aligned}
\small
    \boldsymbol A^\dashv = \mathrm{softmax}(\boldsymbol A) &&
    \boldsymbol A^\vdash = \mathrm{softmax}(\boldsymbol A^T)
\end{aligned}
\end{equation}


\subsection{Hybrid Message Fusion} \label{sec:hybrid}
To better incorporate the information of the static graph and the dynamic graph, we propose a novel Hybrid Message Passing GNN (HMP-GNN), which are performed on both semantic-based static graph and attention-based dynamic graph.

\textbf{Static Message Passing.} 
Since the semantics-based static graph is a directed and unweighted graph, we opt to employ a bidirectional message passing GNN~\cite{chen2019reinforcement} to encode the graph.
% To learn the static graph representation from node embeddings $comp$ returned by complementary-graph mechanism, a bidirectional message passing approach~\cite{chen2019reinforcement} is applied.
Specifically, for every node $v$ at each computation hop $k$, where $\boldsymbol h_v^0 \in \boldsymbol {comp}$, we apply a simple mean aggregation function that takes as input a set of incoming/outgoing neighboring node embeddings computed from the previous hop, and outputs a backward/forward aggregated vector $\boldsymbol h_{\mathcal{N}_{\dashv(v)}}^k$ / $\boldsymbol h_{\mathcal{N}_{\vdash(v)}}^k$. Then we fuse the above two aggregated vectors via a fusion function.
\begin{equation}
\begin{gathered}
\small
  \boldsymbol h_{\mathcal{N}_{\dashv(v)}}^k = \mathrm{SUM}(\{\boldsymbol h_u^{k-1} + \boldsymbol e_{v, u}, \forall u \in \mathcal{N}_{\dashv(v)} \}) \qquad
  \boldsymbol h_{\mathcal{N}_{\vdash(v)}}^k = \mathrm{SUM}(\{\boldsymbol h_u^{k-1}+ \boldsymbol e_{v, u}, \forall u \in \mathcal{N}_{\vdash(v)} \})  \\
  \boldsymbol h_{sta}^k = \mathrm{Fuse}(\boldsymbol h_{\mathcal{N}_{\dashv(v)}}^k, \boldsymbol h_{\mathcal{N}_{\vdash(v)}}^k)
 \end{gathered}
\end{equation}
 Here the fusion function is designed as a gated sum of two inputs.
 \begin{equation}
 \label{func:fusion}
 \begin{aligned}
 \small
 \mathrm{Fuse(\boldsymbol a,\boldsymbol b)} = \boldsymbol z \odot \boldsymbol a + (1-\boldsymbol z) \odot \boldsymbol b & & \boldsymbol z= \sigma(\boldsymbol W_z[\boldsymbol a;\boldsymbol b;\boldsymbol a \odot \boldsymbol b; \boldsymbol a- \boldsymbol b ] +\boldsymbol b_z)
 \end{aligned}
 \end{equation}
 where $\odot$ is the component-wise multiplication, $\sigma$ is a sigmoid function and $z$ is a gating vector.

\textbf{Dynamic Message Passing.} \label{sec: dynamic}
The node and edge information is propagated on the attention-based dynamic graph with the normalization adjacency matrices $\boldsymbol A^\dashv$ and $\boldsymbol A^\vdash$, defined as
 \begin{equation}
 \begin{aligned}
 \small
 \boldsymbol h_{v^\dashv}^k = \sum_{j=1}^m \boldsymbol A^{\dashv}_{v,j}(\boldsymbol h_j^{k-1}\boldsymbol W^V + \boldsymbol e_{v,j} \boldsymbol W^F) & &
 \boldsymbol h_{v^\vdash}^k = \sum_{j=1}^m \boldsymbol A^{\vdash}_{v,j}(\boldsymbol h_j^{k-1}\boldsymbol W^V + \boldsymbol e_{v,j}\boldsymbol W^F)
 \end{aligned}
 \end{equation}
where $\boldsymbol h_j^0 \in \boldsymbol {comp}$, $m$ is the total number of nodes and $k$ is the computation hop. Finally, we obtain dynamic aggregated vectors $\boldsymbol h_{dyn}^k$ by feeding $\boldsymbol h_{v^\dashv}^k$ and $\boldsymbol h_{{v^\vdash}}^k$ with fusion function defined in~\cref{func:fusion}.


\textbf{Hybrid Message Passing.}\label{sec:hybrid}
Given the static/dynamic aggregated vectors $\boldsymbol h_{sta}^k$/$\boldsymbol h_{dyn}^k$ for static and dynamic graphs, respectively, we fuse both vectors and feed the resulting vector to a Gated Recurrent Unit (GRU) to update node representations.
 \begin{equation}
 \begin{small}
 \begin{aligned}
 \boldsymbol h_v^k =\mathrm{GRU}(\boldsymbol h_v^{k-1}, \mathrm{Fuse}(\boldsymbol h_{sta}^k, \boldsymbol h_{dyn}^k))
 \end{aligned}
 \end{small}
 \end{equation}
 After $n$ hops of GNN computation, we obtain the final node representation $\boldsymbol h_v^n$ and then apply max-pooling over all nodes $\{\boldsymbol h_v^n, \forall v \in V \}$ to get a $d$-dim graph representation $\boldsymbol h^g$.


\subsection{Decoder}
The decoder is similar with other state-of-the-art Seq2seq models~\cite{bahdanau2014neural,luong2015effective} where an attention-based BiLSTM decoder is used. The decoder takes the graph-level representation $\boldsymbol h^g$ as initial hidden states and concatenate the node representations with retrieved summary representations $\{\boldsymbol h_v^n, \forall v \in V \} \cup \{\boldsymbol h_{s'_i}, \forall s'_{i} \in s'\}$ as the attention memory and generate the summary.
\subsection{Training and Inference}
We train the model with regular cross-entropy loss, defined as $\mathcal{L} = \sum_t - \mathrm{log} P(s_t^\ast | V, s', s_{<t}^\ast)$, where $s_t^\ast$ is the word at the $t$-th position of the ground-truth. To alleviate the exposure bias, we utilize schedule teacher forcing~\cite{bengio2015scheduled}. During the inference, we use beam search to generate final results.

